ToReMi: Topic-Aware Data Reweighting for Dynamic Pre-Training Data Selection

Pre-training large language models (LLMs) necessitates enormous diverse textual corpora, making effective data selection a key challenge for balancing computational resources and model performance. Current methodologies primarily emphasize data quality metrics and mixing proportions, yet they fail to adequately capture the underlying semantic connections between training samples and quality disparities within individual domains. We introduce ToReMi (Topic-based Reweighting for Model improvement), a novel two-stage framework that dynamically adjusts training sample weights according to their topical associations and observed learning patterns. Our comprehensive experiments reveal that ToReMi variants consistently achieve superior performance over conventional pre-training approaches, demonstrating accelerated perplexity reduction across multiple domains and enhanced capabilities on downstream evaluation tasks. Code is available at https://github.com/zxx000728/ToReMi.

==> latex/texes/01.Introduction.00.en.tex <==
\begin{figure}[t]
\centering
\resizebox{\columnwidth}{!}{
\includegraphics[width=1\linewidth]{latex/figs/framework.pdf}
}
\caption{
The framework of ToReMi, a two-stage, topic-based reweighting method for dynamic pre-training data selection and model improvement.
During each training interval, training samples are reweighted based on their topic labels and previous training dynamics.
}
\label{fig:framework}
% \vspace{-3mm}
\end{figure}

% Background
The pre-training datasets~\citep{gao2020pile, soldaini2024dolma, penedo2023refinedweb} for large language models (LLMs) are typically composed of vast amounts of unannotated text data, sourced from diverse origins with varying quality.
As the scale of model parameters and pre-training datasets continues to grow~\citep{kaplan2020scalinglawsneurallanguage, hoffmann2022trainingcomputeoptimallargelanguage}, pre-training has become the most computationally intensive phase of model training, while also determining the foundational knowledge embedded in the model~\citep{zhou2023limaalignment}.
To reduce computational costs and enhance knowledge, data selection has become increasingly critical in training high-quality LLMs.

Existing data selection methods primarily focus on two key aspects: data quality and data mixing.
Mainstream preprocessing workflows typically involve language filtering, deduplication, and denoising to ensure quality~\citep{soldaini2024dolma, penedo2023refinedweb, albalak2024survey}.
Data quality is often evaluated using rule-based heuristics and classifiers~\citep{raffel2023exploring, rae2022scaling, longpre2023pretrainers}, or proxy models to measure similarity to high-quality reference distributions~\citep{xie2023data, wenzek2019ccnet}.
Data mixing then optimizes the dataset by adjusting domain ratios~\citep{xie2023doremi, du2022glam} or employing diverse sampling strategies~\citep{soldaini2024dolma, thrush2024improvingpretrainingdatausing}, thereby enhancing the model's generalization and task-specific performance.

% Motivation
Despite advancements in improving LLM pre-training efficiency, identifying the optimal subset of pre-training data remains challenging.
For data quality, (1) heuristic or classifier-based methods focus on surface features, failing to capture the latent semantic relationships within the corpus.
(2) The static nature of manual rules hinders their ability to adapt to training dynamics, making them prone to mismatched selections.
(3) Offline methods, such as training proxy models, are computationally expensive and rely on predefined data distributions, which restricts generalization.
For data mixing, current methods emphasize inter-domain ratios (e.g., Web, Books) but ignore quality differences within domains.
As a result, a key question arises: \textbf{How to dynamically select high-quality data during pre-training while accounting for both the corpus's semantic relationships and within-domain quality differences?}

% Method
To address these challenges, we propose a two-stage \textbf{To}pic-based \textbf{Re}weighting framework for \textbf{M}odel \textbf{i}mprovement (\textbf{ToReMi}).
Topics, as abstractions of high-level semantics, capture semantic relationships within the corpus and enable fine-grained distinctions within the domains.
Moreover, topics serve as a valuable basis for evaluating data quality, as themes like academic papers often indicate high-quality content, whereas social media generally suggests lower quality.
Based on this, ToReMi adjusts sample weights across topics based on the model's training dynamics, enabling the selection of high-quality data during pre-training.
In the first stage, greater weights are assigned to challenging samples to facilitate efficient knowledge acquisition.
In the second stage, noisy samples are downweighted to minimize interference, while valuable samples are prioritized to enhance the retention of critical information.

Extensive experiments were conducted and key findings include:
(1) All ToReMi variants reduce perplexity faster and achieve lower final scores than standard pre-training across domains, demonstrating faster convergence and better language modeling capability.
(2) ToReMi shows task-dependent improvements on downstream tasks, particularly for syntactic understanding and sentiment analysis.
(3) In synthetic noise experiments, our two-stage approach effectively mitigates the impact of noisy data through downweighting in later training.
(4) Ablation studies reveal the importance of optimizing transition timing and weight bounds to balance early aggressive learning with later noise reduction.

% % Contribution
% Our contributions are summarized as follows:
% (1) We propose a two-stage data reweighting framework based on corpus topics, which adaptively adjusts the weights of samples across different topics during pre-training to enable dynamic data selection.

==> latex/texes/01.Introduction.00.zh.tex <==
% Background
预训练数据集通常由大量未标注的文本数据构成，这些文本来源多样且质量不一。
随着模型参数规模和预训练数据集不断扩大，预训练占据了模型训练的大部分计算资源，同时决定着模型的基础知识储备。
为了降低计算成本并提升模型的知识水平，数据选择在训练高质量的LLM中显得愈发重要。

现有的数据选择方法主要聚焦于两个关键因素：语料质量和数据配比。
为了构建高质量的预训练数据集，主流的数据预处理流程通常包括语言筛选、去重和去噪等步骤。
语料质量的评估通常依赖人工设计的规则或分类器，或通过训练代理模型来衡量语料与高质量参考数据的相似性。
在此基础上，数据配比通过调整不同领域数据的混合比例或采用多样化的采样策略，进一步提升模型的泛化能力及在特定任务中的表现。

% Motivation
尽管这些方法显著提升了LLM预训练的效率，寻找预训练数据的最佳子集仍面临以下挑战。
对语料质量而言，
(1) 基于规则或分类器的方法通常聚焦于表层特征，难以捕捉语料间的潜在语义关联。
(2) 人工设计的规则无法根据模型在预训练过程中的表现动态调整筛选标准，导致筛选结果难以适应模型的实际需求。
(3) 训练代理模型等离线策略成本高昂，需要预定义理想语料分布，限制了模型的泛化能力。
对数据配比而言，现有数据混合方法主要关注领域间的配比 (e.g., Web, Book)，对同领域内的语料往往采用统一处理，忽略了领域内语料的质量差异。
由此引发了一个值得探索的科研问题：如何在预训练过程中动态选择高质量数据，既关注语料间的语义关联，又有效区分其质量差异？

% (1) 基于规则的方法通常聚焦于表层特征（如字符数、句子长度等），难以捕捉语料间的潜在语义关联。且规则是静态的，无法根据模型在预训练过程中的表现动态调整筛选标准，导致筛选结果可能与实际训练需求不完全匹配。
% (2) 基于分类器的方法通常对单一样本进行评分，未能充分利用样本间的关系信息进行整体优化，且分类器的训练数据质量将直接影响筛选结果。

% Method
为了解决上述问题，我们引入语料主题作为特征，并提出了一种高效的两阶段数据重加权框架，用于在预训练过程中动态选择高质量数据。
主题作为语料高层语义的抽象，能够准确反映文本的核心内容。
同一主题下的文本在语义上具有较高的一致性，有助于建立语料之间的语义联系。
相比传统的领域划分，主题可以在更细粒度上区分同一领域内的语料，从而提供更丰富的语义信息。
我们提出的两阶段框架基于模型在预训练过程中的动态表现，自适应调整不同主题样本的权重。
在第一阶段，对潜在的难样本赋予更高权重，帮助模型快速学习新知识；在第二阶段，降低潜在噪音样本的权重，以减少干扰，同时提高有效知识的权重，进一步强化模型对关键知识的掌握。
使用该框架从头预训练GPT-2，实验结果表明模型收敛速度显著提升，同时在xxx任务上表现优异，达到xxx效果。

% 为了解决上述问题，我们引入语料主题作为特征进行数据选择。
% 主题作为语料高层语义的抽象，能够反映文本的核心内容。同一主题下的文本通常在语义上具有较高的一致性，可帮助建立语料间的语义联系。
% 相较于领域划分，主题可按不同粒度更细致地区分同领域内的语料。例如，Wiki语料中的科技和金融主题可以进一步细分为机器学习、区块链等子主题。通过调整主题粒度，可以实现更精细的数据选择。
% 此外，主题特征还能辅助评估语料质量。例如，学术论文等主题通常对应高质量语料，而社交媒体内容等主题则可能质量较低，这为数据选择提供了重要依据。
% % reweighting进行数据选择
% 为实现基于语料主题在预训练过程中动态选择高质量数据，我们提出了一种高效的两阶段数据重加权框架。该框架根据模型在训练过程中的表现，自适应调整不同主题样本的权重，从而强化有效知识的学习，同时减少噪音干扰。
% 方法效果

% Contribution
我们的贡献总结如下：
(1) 基于语料主题进行数据选择，提出了一个两阶段的数据重加权框架，在训练过程中自适应调整不同主题样本的权重，实现动态数据选择。
(2) Some findings


==> latex/texes/01.Introduction.01.tex <==
大型语言模型（LLMs）的预训练数据集通常由海量文本数据构成，这些数据来源多样且质量参差不齐。
随着模型参数规模和预训练数据集容量的持续扩大，预训练阶段已成为模型训练过程中最为关键的环节，它直接决定了模型所掌握的基础知识结构和推理能力。
因此，科学地选择和优化预训练数据已成为构建高性能LLMs的核心技术挑战。

现有的数据选择方法主要聚焦于两个关键维度：数据质量评估和数据混合策略。
这两种方法的根本目标都是甄别并保留对模型训练最具价值的数据，同时剔除可能引入干扰的低质量样本。
标准的预处理工作流程通常包含语言识别与过滤、重复内容移除以及噪声数据清理等步骤，以确保基本的数据质量。
质量评估环节主要依赖于基于规则的启发式方法和监督式分类器进行筛选，而数据混合则通过精心设计的领域比例调整和多样化采样策略来优化语料结构，以增强模型的泛化能力和在特定任务上的表现。

然而，构建最优预训练数据集仍然面临诸多理论和实践挑战。
在数据质量评估领域，基于规则和分类器的方法本质上受限于标注者的主观判断和有限的训练数据，这使得它们在识别复杂的质量差异上能力有限，通常只能有效过滤那些明显低质的样本。
在数据混合策略方面，当前方法往往采用较为粗放的方式，主要通过调整不同主题或领域类别的语料比例来验证配比效果，缺乏对数据内在语义关系和动态训练需求的深入考量。
这些局限共同制约了预训练效率的提升和模型性能的优化。

针对上述挑战，我们提出一个核心研究问题：
如何在预训练过程中动态选择高质量数据，同时考虑语料库的潜在语义关系和领域内部的质量变化？
为解决这一问题，我们开发了一个两阶段的Topic-based Reweighting Framework for Model Improvement (ToReMi）。
ToReMi的核心创新在于其基于主题类别的集体权重调整机制。
根据训练过程中每个主题类别内所有样本的集体表现，动态调整整个主题类别的权重。
具体而言，ToReMi分为两个关键阶段：
(1) 在初始训练阶段，系统为表现出较高学习难度的主题类别分配更高权重，促使模型优先攻克这些具有挑战性的内容；
(2) 在后续训练阶段，系统逐步降低训练表现不佳的主题类别权重以减少负面干扰。
通过这种基于主题的集体调整策略，ToReMi能够在不增加额外计算开销的前提下，有效优化整体预训练数据分布，并根据主题的权重为开发人员提供各主题对模型训练影响的可解释性分析。

为全面验证ToReMi的有效性，我们基于GPT-2架构进行了系统实验。
实验数据集由2.6B tokens的精选Wikipedia语料构成，并通过大型语言模型的标注将其划分为39个主题类别。
实验结果表明，ToReMi方法在Paloma评估语料上的log perplexity测试中，全面优于标准预训练方法和强化噪声防御的基线方法。
特别值得注意的是，在人为注入噪声的实验环境中，ToReMi在GLUE基准测试上比标准预训练方法平均提升了1.9\%的性能。
进一步的稳健性分析显示，即使在不同超参数配置下，ToReMi仍能稳定优于基线预训练方法。

% 针对上述问题，我们提出一个关键问题：
% 如何在预训练过程中动态选择高质量数据，同时考虑语料库的语义关系和领域内的质量变化？
% 为解决这一问题，我们开发了一个两阶段基于主题的重加权框架用于模型改进（ToReMi）。
% 该框架利用主题作为高级语义抽象，不仅能捕捉语料库内的语义关联，还能实现领域内部的细粒度区分。
% ToReMi根据模型的训练动态调整样本权重：
% 在第一阶段，优先学习具有挑战性的样本以高效获取知识；
% 在第二阶段，降低噪声样本的权重以减少干扰，同时保留价值高的样本以巩固关键知识。
% 通过这种方式，ToReMi能够在不增加任何计算开销的前提下，根据训练情况动态优化预训练数据的使用，提高模型训练效率和最终性能，同时还能将主题标签的权重反馈给开发者，让开发者知悉哪个主题会影响训练的进行。

% 我们使用了在GPT-2上验证了ToReMi方案，并从清洗过的Wikipedia语料中采样2.6B，通过大模型标注分了39个主题。
% 相较于标准预训练，以及加强对于噪音样本学习的防范。
% ToReMi方法在使用Paloma语料用log perplexity测试效果时，全面好过这两种预训练方案。
% 而在人为注入噪音之后，ToReMi的方法能够在GLUE数据集上取得比标准预训练要好上1.9\%的效果，以及在任意调整超参数的情况下，都能够稳定地好于baseline预训练方法。


==> latex/texes/01.Introduction.02.tex <==
Pre-training datasets for large language models (LLMs) typically comprise vast amounts of text data from diverse sources with varying quality levels~\citep{gao2020pile, soldaini2024dolma, penedo2023refinedweb}. 
As model parameter scale and pre-training dataset capacity continue to expand~\citep{kaplan2020scalinglawsneurallanguage, hoffmann2022trainingcomputeoptimallargelanguage}, the pre-training phase has become the most critical component in LLM development, directly determining the foundational knowledge and reasoning capabilities embedded within the model~\citep{zhou2023limaalignment}. 
Consequently, the scientific selection and optimization of pre-training data has emerged as a core technical challenge in constructing high-performance LLMs.

Existing pre-training data selection methodologies primarily focus on two key dimensions: 
data quality assessment and data mixing strategies. 
The aim of both approaches is to identify and retain the most valuable data for pre-training while eliminating potentially disruptive low-quality samples. 
Standard preprocessing workflows typically include language identification, corpora filtering, duplicate content removal, and noise reduction procedures to ensure corpora quality~\citep{soldaini2024dolma, penedo2023refinedweb, albalak2024survey}. 
Quality assessment predominantly relies on rule-based heuristics and supervised classifiers for screening~\citep{raffel2023exploring, rae2022scaling, longpre2023pretrainers}, while data mixing optimizes corpus structure through carefully designed domain ratio adjustments and diverse sampling strategies~\citep{xie2023doremi, du2022glam, soldaini2024dolma, thrush2024improvingpretrainingdatausing} to enhance model generalization and task-specific performance.

Despite these advances, constructing optimal pre-training datasets still faces numerous theoretical and practical challenges. 
In the domain of quality assessment, rule-based and classifier-driven methods are inherently limited by annotators' subjective judgments and restricted training data, rendering them capable of effectively filtering only obviously low-quality samples, while struggling to identify more nuanced quality variations~\citep{wenzek2019ccnet, xie2023data}. 
Regarding data mixing strategies, current approaches often employ relatively coarse methods, primarily validating mixture effectiveness by adjusting proportions across different topics or domain categories, lacking deeper consideration of intrinsic semantic relationships within the data and dynamic training requirements~\citep{xie2023doremi, du2022glam}. 
These limitations collectively constrain improvements in pre-training efficiency and model performance optimization.

To address these challenges, we propose a central research question: 
How can we dynamically select high-quality data during pre-training while accounting for both latent semantic relationships within the corpus and quality variations within domains?
To address these challenges, we propose a two-stage \textbf{To}pic-based \textbf{Re}weighting framework for \textbf{M}odel \textbf{i}mprovement (\textbf{ToReMi}).
The core innovation of ToReMi lies in its collective weight adjustment mechanism based on topic categories. 
Rather than optimizing weights for individual samples, it dynamically adjusts the weight of entire topic categories based on the collective performance of all samples within each topic during training. 
Specifically, ToReMi operates in two critical phases: 
(1) During the initial training phase, the system assigns higher weights to topic categories exhibiting greater learning difficulty, encouraging the model to prioritize mastering these challenging knowledge domains; 
(2) In the subsequent training phase, the system gradually reduces the weights of poorly performing topic categories (potentially containing more noise) to minimize negative interference. 
Through this topic-based collective adjustment strategy, ToReMi effectively optimizes the overall pre-training data distribution without incurring additional computational costs while providing developers with interpretable analysis of how different topics impact model training through topic weight feedback.

To comprehensively validate ToReMi's effectiveness, we conducted systematic experiments using the GPT-2 architecture~\citep{raffel2023exploring, rae2022scaling}. 
The experimental dataset comprised 2.6B tokens of curated Wikipedia content, categorized into 39 semantic topics through large language model annotation. 
Results demonstrate that the ToReMi method comprehensively outperforms both standard pre-training approaches and enhanced noise-resistant baselines in log perplexity tests on the Paloma evaluation corpus~\citep{gao2020pile}. 
Notably, in experiments with artificially injected noise, ToReMi achieved an average 1.9\% performance improvement on GLUE benchmarks compared to standard pre-training~\citep{longpre2023pretrainers}. 
Further robustness analysis reveals that ToReMi consistently outperforms baseline pre-training methods across different hyperparameter configurations, demonstrating exceptional methodological stability and adaptability.

==> latex/texes/07.Limitation_EthicalConcern.00.tex <==
\section{Limitation}
This is the limitation section.

\section{Ethical Concern}
This is the ethical concern section.

